muPRL: A Mutation Testing Pipeline for Deep Reinforcement Learning based on Real Faults

Reinforcement Learning (RL) is increasingly adopted to train agents that can deal with complex sequential tasks, such as driving an autonomous vehicle or controlling a humanoid robot. Correspondingly, novel approaches are needed to ensure that RL agents have been tested adequately before going to production. Among them, mutation testing is quite promising, especially under the assumption that the injected faults (mutations) mimic the real ones. In this paper, we first describe a taxonomy of real RL faults obtained by repository mining. Then, we present the mutation operators derived from such real faults and implemented in the tool muPRL. Finally, we discuss the experimental results, showing that muPRL is effective at discriminating strong from weak test generators, hence providing useful feedback to developers about the adequacy of the generated test scenarios.

==> operator.tex <==
\begin{table*}[]
\caption{Comparing our Mutation Operators with Prior Work}
\scalebox{0.65}{
\begin{tabular}{rp{7cm}p{9cm}p{9cm}}
\toprule
 Index &                                                          Mutation Operator &                                                                                                                                                                                                                            Description &                                                                                                          Reason for keeping/dropping \\
\midrule
     1 &                                                               Reward Noise &                                                                                                                                                                                     The reward recieved by the environment is modified &                                                                           Corresponds to the bug label, "Suboptimal Reward Function" \\
     2 &                                                    Mangled/ Random/ Repeat & The new state and the its corresponding reward are unrelated/ The new state and its corresponding reward aren't related to the action taken/ The previous state and its corresponding reward is returned during the current time step  &                                                                                 Mutation operator cannot be mapped to a RL framework \\
     3 &                                                         No discount factor &                                                                                                                                                                      The discount factor isn't used while computing the sum of rewards &                                                                           Corresponds to the bug label, "Suboptimal discount factor" \\
     4 &                                                                 No reverse &                                                                                                                                                                                           The rewards are summed in the opposite order &                                                                                 Mutation operator cannot be mapped to a RL framework \\
     5 &                                                       Missing state update &                                                                                                                                                                              The agent's observations aren't updated after a time step &                                                                                 Mutation operator cannot be mapped to a RL framework \\
     6 &                                                     Missing terminal state &                                                                                                                                                                         The conditional for checking if a state is terminal is mutated & Corresponds to the bug labels, "Flags indicating successful termination or timeout not set properly " and "Missing check for dones " \\
     7 & Incorrect loss function/ Policy activation change/ Policy optimizer change &             A incorrect loss is utilized for deep reinforcement learning algorithm/ The activation function for the deep reinforcement learning agent is modified/ The optimizer for the deep reinforcement learning agent is modified &                                                                                           Mutation operator is a Deep Learning Fault \\
     8 &                      Reward Reduction/ Reward Increase/ Reward Instability &                                                                                                                                                     Lower large reward values/ Increase smaller reward values/ Generate random rewards &                                                                           Corresponds to the bug label, "Suboptimal Reward Function" \\
     9 &             State Record Crash/ State Delay/ State Repetition/ State Error &                          Drop or increase state-action pairs/ The state is associated with an action taken at a later time step*/ The state is fixed with continous actions/ Break the association between a state and its action pair &                                                                                 Mutation operator cannot be mapped to a RL framework \\
    10 &                                                                         QF &                                                                                                                                                                                                                  The Q-Table is fuzzed &                                                                                 Mutation operator cannot be mapped to a RL framework \\
    11 &                                                              INR/ OND/ ONA &                                                                                                                                                         Input neurons are dropped/ Output neurons are dropped/ Ouput neurons are added &                                                                                           Mutation operator is a Deep Learning Fault \\
    12 &                                                       Changing Exploration &                                                                                                                                                         Switch exploration strategies between epsilon greedy and jittering parameters  &                                                                                      Did not find evidence of this bug in a taxonomy \\
    13 &                                                           Mutating Epsilon &                                                                                                                                                                                                 Mutating the value of epsilon operator &                                                               Corresponds to the bug label, "Suboptimal exploration rate - Epsilon " \\
    14 &                                                             Changing Noise &                                                                                                                                                                                     The method of jittering the parameters is modified &                         Corresponds to the bug labels, "Suboptimal application of dirichilet noise" and "Suboptimal noise sampling"  \\
    15 &                                           Switching Buffer/ Fuzzing Buffer &                                                                                                                                                                   The replay buffer is turned off/ The replay buffer values are fuzzed &                                                                                 Mutation operator cannot be mapped to a RL framework \\
    16 &                                                  Shuffling Replay Priority &                                                                                                                                                                             The replay frequency of significant experiences is reduced &                                                              Corresponds to the bug label, "Suboptimal sampling from replay buffer"  \\
    17 &                                                         Precision Mutation &                                                                                                                                                                     The precision by which continous spaces are discretized is mutated &                                                                              Corresponds to the bug label, "Suboptimal state space " \\
    18 &                                                     Approximation Mutation &                                                                                                                                                                                          Function approximation algorithms are mutated &                                Corresponds to the bug label, "Use of inappropriate function approximator for the\textbackslash ngiven environment" \\
\bottomrule
\end{tabular}
}
\label{demo-table}
\end{table*}


